Step-by-Step Diffusion: An Elementary Tutorial

We present an accessible first course on diffusion models and flow matching for machine learning, aimed at a technical audience with no diffusion experience. We try to simplify the mathematical details as much as possible (sometimes heuristically), while retaining enough precision to derive correct algorithms.

==> app_scratch.tex <==










==> sec_ddim_proof_old.tex <==
\newcommand{\rG}{{G_t}[x_0]}
\newcommand{\va}{v_t[a]}
\newcommand{\vb}{v_t[b]}
\newcommand{\vxn}{v_t[x_0]}


We will now show a \emph{deterministic}
reverse sampler for Gaussian diffusion---
which appears similar to the stochastic sampler
of the previous section, but is conceptually quite different.
This sampler is equivalent to the ``DDIM update,''
in our simplified setting.

We consider the same Gaussian diffusion setup as the previous section,
with the joint distribution $(x_0, x_\dt, \dots, x_1)$
and conditional expectation function
$\mu_{t}(z) := \E[x_{t} \mid x_{t+\dt} = z].$
The reverse sampler is defined below, and listed explicitly in Pseudocode~\ref{alg:ddim_inf}.

\begin{mdframed}[nobreak=true]
\underline{Algorithm 2: Deterministic Reverse Sampler (DDIM-like)}\\
For input sample $x_t$, and step index $t$, output:
\begin{align}
\label{eqn:ddim}
    \hat{x}_{t-\dt} \gets
    x_t + \lambda({\mu}_{t-\dt}(x_t) - x_t)
\end{align}
where $\lambda := \left( \frac{\sigma_{t}}{\sigma_{t-\dt}+ \sigma_{t}} \right )$
and $\sigma_t \equiv \sigma_q \sqrt{t}$ 
from Equation~\eqref{eqn:intro-xt-dt}.
\end{mdframed}

How do we show that this defines a valid reverse sampler?
Since Algorithm 2 is \emph{deterministic},
it does not make sense to argue that it \emph{samples}
from $p(x_{t-\dt} \mid x_t)$, as we argued for the DDPM-like stochastic sampler.
Instead, we will directly show that Equation~\eqref{eqn:ddim}
implements a valid \emph{transport map}
between the marginal distributions $p_{t}$ and $p_{t-\dt}$.
That is, if we let $F_t$ be the update of Equation~\eqref{eqn:ddim}:
\begin{align}
    F_t(z) :=& ~z + \lambda(\mu_{t-\dt}(z) - z)\\
    =& ~z + \lambda(\E[x_{t-\dt} \mid x_t = z] - z)
\label{eqn:ddim_F}
\end{align}
then we want to show that\footnote{
The notation $F\sharp p$ means the
distribution of $\{F(x)\}_{x \sim p}$.
This is called the \emph{pushforward}
of $p$ by the function $F$.}
\begin{align}
F_t \sharp p_t \approx p_{t-\dt}.
\end{align}


{\bf Proof overview:}
The usual way to prove this
is to use tools from stochastic calculus, but 
we'll present an elementary derivation.
Our strategy will be to first show that Algorithm 2 is correct
in the simplest case of a point-mass distribution,
and then lift this result to full distributions
by marginalizing appropriately.
For the experts, this is similar to ``flow-matching'' proofs.

\subsection{Case 1: Single Point}
Let's first understand the simple case where 
the target distribution $p_0$ is a single point mass in $\R^d$.
Without loss of generality\footnote{Because we can just ``shift'' our coordinates to make it so. Formally, our entire setup including Equation~\ref{eqn:ddim_F} is translation-symmetric.},
we can assume the point is at $x_0 = 0$.
Is Algorithm 2 correct in this case?
To reason about correctness, we want to consider
the distributions of $x_t$ and $x_{t-\dt}$ for arbitrary step $t$.
Then, at step $t$, the relevant random variables are:
\begin{align*}
    x_0 &= 0 \quad\textrm{(deterministically)} \\
    x_{t-\dt} &\sim  \cN(x_0, \sigma_{t-\dt}^2) \\
    x_t &\sim  \cN(x_{t-\dt}, \sigma_{t}^2-\sigma_{t-\dt}^2)
\end{align*}

The marginal distribution of $x_{t-\dt}$ is $p_{t-\dt} = \cN(0, \sigma_{t-1}^2)$,
and the marginal distribution of $x_t$ is $p_t = \cN(0, \sigma_t^2)$.

Let us first find \emph{some} deterministic function $G_t: \R^d \to \R^d$,
such that
$G_t \sharp p_t = p_{t-\dt}$.
There are many possible functions which will work\footnote{For example,
we can always add a ``rotation'' around the origin to any valid map.}, but 
this is the obvious one:
\begin{align}
\label{eqn:gg}
    G_t(z) &:= \left(\frac{\sigma_{t-\dt}}{\sigma_t}\right) z.
\end{align}

The function $G_t$ above simply re-scales the Gaussian distribution of $p_t$,
to match variance of the Gaussian distribution $p_{t-\dt}$.
It turns out this $G_t$ is exactly equivalent to the
step $F_t$ taken by Algorithm 2,
which we will now show.

\anote{
Can we go `directly' from \ref{eqn:gg} to a proof of DDIM, assuming we have the flow stuff? 
First, I want to derive the pointwise flow directly from $G$:
\begin{align}
    G_t(x_t) &:= \left(\frac{\sigma_{t-\dt}}{\sigma_t}\right) x_t 
    = \sqrt{1 - \frac{\dt}{t}} x_t 
    \approx (1 - \frac{\dt}{2})x_t \\
    \implies v_t(x_t) &\approx -\frac{x_{t-\dt} - x_t}{\dt} \equiv -\frac{G_t(x_t) - x_t}{\dt}
    = \frac{1}{2} x_t
\end{align}
Putting the $x_0$ back (which was assumed to be zero) we get the pointwise flow:
$$\Tab{x_1}{x_0}_t(x_t)= \frac{1}{2} (x_t - x_0)$$.
Now, we just apply the marginal flow machinery to get the result.
}


\begin{claim}
    When the target distribution is a point mass $p_0 = \delta_0$,
    then update $F_t$ (as defined in Equation~\ref{eqn:ddim_F})
    is equivalent to the scaling $G_t$ (as defined in Equation~\ref{eqn:gg}):
    \[
    F_t \equiv G_t.
    \]
Thus Algorithm 2 defines a valid reverse sampler for target distribution
$p_0 = \delta_{0}.$
\end{claim}

\begin{proof}
To apply $F_t$, we need to compute
$\E[x_{t-\dt} \mid x_t]$ for our simple distribution.
Since $(x_{t-\dt}, x_t)$ are jointly Gaussian, this is\footnote{Recall
the conditional expectation of two jointly Gaussian random variables $(X, Y)$ is 
$\E[X \mid Y = y] = \mu_X + \frac{\sigma_{XY}}{\sigma_Y^2}(y-\mu_Y)$.
Since $X = x_{t-\dt}$ and $Y = x_t$ are centered at $0$, we have $\mu_X=\mu_Y=0$.
For the covariance term,
since $x_t = x_{t-\dt} + \eta$ we have $\E[x_t x_{t-\dt}] = \E[x_{t-\dt}^2] = \sigma_{t-\dt}^2$.
}
\begin{align}
\label{line:exp}
    \E[x_{t-\dt} \mid x_t]
    &= \left(\frac{\sigma_{t-\dt}^2}{\sigma_t^2}\right) x_t.
\end{align}


The rest is just algebra:
\begin{align*}
    F_t(x_t) &:= x_t + \lambda(\E[x_{t-\dt} \mid x_t ] - x_t)  \mathnote{by definition of $F_t$}\\
    &= 
    x_t + \left( \frac{\sigma_{t}}{\sigma_{t-\dt}+ \sigma_{t}}  \right)
    (\E[x_{t-\dt} \mid x_t ] - x_t) \mathnote{by definition of $\lambda$}\\
    &= 
    x_t + \left( \frac{\sigma_{t}}{\sigma_{t-\dt}+ \sigma_{t}}  \right)
    \left(\frac{\sigma_{t-\dt}^2}{\sigma_t^2} - 1\right)x_t \mathnote{by Line~\eqref{line:exp}}\\
    &= \left(\frac{\sigma_{t-\dt}}{\sigma_t}\right) x_t \mathnote{by algebra} \\
    &= G_t(x_t).
\end{align*}
We therefore conclude that Algorithm 2
is a correct reverse sampler,
since it is equivalent to $G_t$, and $G_t$ is valid.
\end{proof}

The correctness of Algorithm 2 still holds
if $x_0$ is an arbitrary point instead of $x_0 = 0$,
since everything is transitionally symmetric.
To be explicit:
\marginnote{None of the results so far require any limits or approximations; they hold even for large step sizes $\sigma$.}




\begin{claim}
\label{claim:ddim_x0}
\pnote{move to appendix.}
    Suppose the target distribution is a point mass
    at $x_0 \in \R^d$, i.e. $p_0 = \delta_{x_0}$.
    Define the function
\begin{align}
   \rG(x_t) = \left(\frac{\sigma_{t-\dt}}{\sigma_t}\right)(x_t - x_0) + x_0.
\end{align}
Then we clearly have $\rG \sharp p_t = p_{t-\dt}$, and moreover
    \[
    \label{eqn:FtExp}
    \rG(x_t)
    = 
    x_t + \lambda(\E[x_{t - \dt} \mid x_t] - x_t)
    =: F_t(x_t).
    \]
Thus Algorithm 2 defines a valid reverse sampler for target distribution
$p_0 = \delta_{x_0}.$
\end{claim}

\subsection{Velocity Fields}
\label{sec:ddim-vf}
It will be helpful to think of the update $F_t$
as defining a vector field, which assigns each point $x_t \in \R^d$
to its new location $F_t(x_t)$.
The corresponding vector field $v_t$ is the ``movement vector'' of these points,
i.e. the displacement
\begin{align}
v_t(x_t) &:= F_t(x_t) - x_t.
\end{align}
In the setting of Claim~\ref{claim:ddim_x0}, with $p_0=\delta_{x_0}$,
we have
\begin{align}
\label{eqn:vtz}
v_t(x_t) &= \left( \frac{\sigma_{t} - \sigma_{t-\dt}}{\sigma_{t}} \right) (x_0 - x_t).
\end{align}
This is a vector field which always points towards the initial point $x_0$,
as depicted in Figure~\ref{fig:flow_single_pt}.

\begin{marginfigure}
  \includegraphics[width=\linewidth]{figs/flow.pdf}
  \caption{Velocity field $v_t$ of Equation~\eqref{eqn:vtz}, overlaid
  on the Gaussian distribution $p_t$.}
  \caption{}
  \label{fig:flow_single_pt}
\end{marginfigure}


The physical intuition for $v_t$ is: imagine a gas of non-interacting particles,
with density field given by $p_t$. Then, suppose all particles
shift their positions such that a particle at position $z$ shifts by $v_t(z)$.
The resulting gas will have density field $p_{t-\dt}$.

In the limit of small stepsize $\dt$, speaking informally,
we can think of $(v_t / \dt)$ as a \emph{velocity field}---
which specifies the instantaneous velocity
of particles moving according to Algorithm 2.
This velocity field interpretation will be useful for us in the following section.




\subsection{Case 2: Two Points}
  
Now suppose the target distribution is a mixture of two point-masses
at $a, b \in \R^d$:
\[
p_0 := \frac{1}{2}\delta_a + \frac{1}{2}\delta_b.
\]
According to the diffusion process in Equation~\ref{eqn:intro-fwd},
the distribution at time $t$ will be a mixture of Gaussians\footnote{Linearity of the
forward process (with respect to $p^*$) was important here.
That is, roughly speaking, diffusing a distribution
is equivalent to diffusing each individual point in that distribution independently;
the points don't interact.
}:
\[
p_t := \frac{1}{2}\cN(a, \sigma_t^2) + \frac{1}{2}\cN(b, \sigma_t^2).
\]
We now want to show that Algorithm 2 is correct, meaning that
\begin{align}
    F_t \sharp p_t = p_{t-\dt}.
\end{align}

Let us first try to construct \emph{some} function $G_t$
that transforms these distributions correctly, i.e.
such that $G_t \sharp p_t = p_{t-\dt}$.
From the single point case, we know how to do this for each distribution
$\delta_a$, $\delta_b$ \emph{individually}.
To review, for target distribution $\delta_a$ and time step $t$,
we have an associated density field
$A_t := \cN(a, \sigma_t^2)$
and velocity field
$\va$,
such that the velocity transports distributions\footnote{Recall that the velocity field
$\va$ represents the instantaneous velocity of particles from $A_t$ moving towards $a$.}:
\begin{align}
A_t \overset{\va}{\longrightarrow} A_{t-\dt}
\end{align}
From Equation~\eqref{eqn:vtz}, we know 
this velocity field explicitly.
Similarly, when the target distribution is $\delta_b$,
we have associated density and velocity fields $(B_t, \vb)$ such that
\[
B_t \overset{\vb}{\longrightarrow} B_{t-\dt}.
\]

We now want some way of ``combining'' these velocities to yield an overall transport
between $p_t$ and $p_{t-1}$:
\[
\label{eqn:guessT}
\underbrace{\left(\frac{1}{2}A_t + \frac{1}{2}B_t \right)}_{p_t}
\overset{?}{\longrightarrow} 
\underbrace{
\left(
\frac{1}{2}A_{t-\dt} + \frac{1}{2}B_{t-\dt}
\right)}_{p_{t-\dt}}
\]
We may be tempted to just take the average velocity field
$(0.5\va + 0.5\vb)$, but this is incorrect.
To see why, let us revisit the particle interpretation.
If our time-step is small enough\footnote{The time step must be small enough for
the updates to be essentially ``infinitesimal'' steps.
Otherwise, if the step size is large, it may not be possible to combine the two transport
maps with ``local'' (i.e. pointwise) operations alone.},
then our question about how to combine velocities is equivalent to the following 
self-contained question about gasses (illustrated in Figure~\ref{fig:gas}):
\begin{quote}
Suppose we have two colored gasses: A (in red) and B (in blue),
with individual density and velocity fields given by $(A_t, \va)$ and $(B_t, \vb)$
Now suppose we videotape these gases in \emph{grayscale},
so we see all particles as part of one combined-gas.
This combined-gas has apparent density field $C_t := A_t + B_t$.
What is its apparent velocity field?
\end{quote}

\begin{figure*}
    \classiccaptionstyle
    \centering
    \includegraphics[width=0.45\linewidth]{figs/flow_rb.pdf}
    \hfill
    \includegraphics[width=0.45\linewidth]{figs/flow_combo.pdf}
    \caption{Illustration of combining the velocity fields of two gasses.
    Left: The density and velocity fields of two independent gases (in red and blue).
    Right: The effective density and velocity field of the combined gas,
    including streamlines.}
    \label{fig:gas}
\end{figure*}

In the above setting, we can intuitively see that
the effective velocity $v_t^*$ should be a \emph{weighted}-average of the individual gas velocities,
weighted by their densities\footnote{For the experts: to prove this, consider the advection equation
which governs the time-evolution of gas:
\begin{equation}
\label{eqn:advection}
    \frac{\partial}{\partial t} p_t = -\nabla \cdot (p_t v_t)
\end{equation}
Then observe that if both gasses 
individually satisfy this equation,
then so does the combined gas, with our definition of 
combined velocity $v^*_t$.
}.
That is, 
\[
\label{eqn:vel_combo}
v_t^* = \frac{A_t\va + B_t\vb}{A_t+B_t}.
\]





Back to diffusion, the $v_t^*$ above is exactly the velocity field
which transports $p_{t}$ to $p_{t-\dt}$. 
Revisiting Equation~\eqref{eqn:guessT}, we can now say
\[
\underbrace{\left(\frac{1}{2}A_t + \frac{1}{2}B_t \right)}_{p_t}
\overset{v_t^*}{\longrightarrow} 
\underbrace{
\left(
\frac{1}{2}A_{t-\dt} + \frac{1}{2}B_{t-\dt}
\right)}_{p_{t-\dt}}.
\]
We have now solved the main subproblem of this section: we have 
found \emph{one particular}
vector field $v_t^*$ which transports $p_t$ to $p_{t-\dt}$,
for our two-point distribution $p_0$.
It remains to show that this $v_t^*$ is equivalent
to the update of Algorithm 2 (i.e. the function $F_t$ from Equation~\ref{eqn:ddim_F}).




To show this, first notice that the
individual vector field $\va$
can be written as a conditional expectation.
Using the definition\footnote{We add conditioning $x_0 = a$,
because we want to take expectations w.r.t
the two-point mixture distribution,
not the single-point distribution of the previous section.}
of $F_t$ from Equation~\eqref{eqn:ddim_F},
\begin{align}
    \va(x_t) &= F^a_t(x_t) - x_t \\
    &= \lambda \E_{x_0 \sim \delta_a}[ x_{t-\dt} - x_t \mid x_{t} ] \\
    &= \lambda \E_{x_0 \sim \half\delta_a + \half\delta_b} [ x_{t-\dt} - x_t \mid x_0 = a, x_{t} ].
\end{align}
Now the entire vector field $v_t^*$
can be written as a conditional expectation,
because the ``weighting factors'' in our expression for $v^*$
are equivalent to marginalizing $\vxn$ over $x_0 \sim \{a, b\}$.
Explicitly:
\begin{align}
v_t^*(x_t) &=
\va(x_t) \cdot \left(\frac{A_t(x_t)}{A_t(x_t) + B_t(x_t)} \right)
+
\vb(x_t)  \cdot \left(\frac{B_t(x_t)}{A_t(x_t) + B_t(x_t)} \right) \\
&=
\va(x_t) \cdot p(x_0 = a \mid x_t)
+
\vb(x_t) \cdot p(x_0 = b \mid x_t) \mathnote{This should be intuitive:
it weighs vector field $v^a$ by the probability
that $x_t$ was generated by $x_0 = a$.}\\
&=
\lambda \E[ x_{t-\dt} - x_t \mid x_0 = a, x_{t}  ] \cdot p(x_0 = a \mid x_t ) \\
&~+ \lambda \E[ x_{t-\dt} - x_t \mid x_0 = b, x_{t}  ]  \cdot p(x_0 = b \mid x_t ) \\
&=
\lambda \E_{x_0 | x_t}\left[
\E_{x_{t-\dt} \mid x_0, x_t}[ x_{t-\dt} - x_t \mid x_0, x_{t}  ] 
~~\Big|~~ x_t \right]\\
&=
\lambda \E\left[
x_{t-\dt} - x_t \mid x_{t}  
\right]\\
&=: F_t(x_t) + x_t
\end{align}
In the last line, we have observed this exact conditional expectation 
appears in the definition of $F_t$.
Thus, the combined velocity field $v^*_t$ is exactly the velocity
induced by the updates of Algorithm 2,
and so Algorithm 2 is a correct reverse sampler for our two-point mixture distribution.

\subsection{Case 3: Arbitrary Distributions}

Now that we know how to handle two points,
we can generalize this idea to
arbitrary distributions of $x_0$.
At a high level, we observed above that Algorithm 2 respects ``combining'' distributions---
if we know Algorithm 2 works for target distributions $A$ and $B$ individually,
then it will also work for the mixture $\half A + \half B$.
We will not go into details here, because the general proof will be subsumed
by the subsequent section.

It turns out that our overall proof strategy for Algorithm 2 can be generalized
significantly to other types of diffusions, without much work.
This yields the idea of Flow Matching, which we will see in the following section.



==> sec_flows_old.tex <==

\clearpage
\newpage
\section{Flow Matching-old}





We now introduce the framework of Flow Matching \citep{lipman2023flow, ??}.
Flow Matching is a generalization of Gaussian diffusion,
which allows for more flexibility in designing
generative models.
In this section we will first present what is called
\emph{Conditional Flow Matching} \citep{lipman2023flow},
and then generalize further to \emph{Pointwise Flow Matching}.
Pointwise flows include the family of \emph{rectified flows} 
(sometimes called  \emph{linear flows}) 
used by Stable Diffusion 3, for example \citep{liu2022flow,esser2024scaling}.


We have actually already seen the main ideas behind conditional flow matching,
in our analysis of DDIM in Section~\ref{sec:ddim}.
At a high level, here is how we constructed a generative 
model in Section~\ref{sec:ddim}:
\begin{enumerate}
    \item First, we defined how to generate a single point.
    Specifically, we constructed vector fields $\{\va\}_t$ which,
    when applied for all time steps, transported
    a standard Gaussian distribution to an arbitrary delta distribution $\delta_a$.
    \item Second, we determined how to combine two vector fields
    into a single effective vector field. This lets us construct 
    a transport from the standard Gaussian to
    \emph{two} points (or, more generally,
    to a \emph{distribution} over points --- our target distribution).
\end{enumerate}
Neither of these steps particularly require the Gaussian base distribution,
or the Gaussian forward process (Equation~\ref{eqn:intro-fwd}).
The second step of combining vector fields 
remains identical for any two arbitrary vector fields, for example.
This leads us to the general technique of conditional flow matching, which we explain below.

\subsection{Notation and Preliminaries}
\label{sec:flow-notation}

We will use the
``discretized continuous time''
notation from Section~\ref{sec:discretization} throughout.
So instead of writing $(x_t, x_{t+1})$ with $t \in \N$, 
we will instead write $(x_t, x_{t+\dt})$ with $t \in [0, 1]$.

A \emph{flow} is
a collection of vector fields indexed by time: $\{v_t\}_{t \in [0, 1]}$,
along with an associated base distribution $q(x)$, such as a standard normal distribution.
Flows transport the base distribution to a target distribution, 
by applying the following iteration
from $t=1$ down to $t=0$:
\begin{align}
x_1 &\sim q\\
x_{t-\dt} &:= x_t + v_t(x_t)\dt \label{eqn:iterx}
\end{align}
For the reader familiar with ODEs, for a fixed $x_1$ the trajectory
of $x_t$ is the solution to the ODE:
\[
\label{eqn:v_ode}
\frac{dx_t}{dt} = -v_t(x_t),
\]
with boundary condition $x_1$.
When $x_1 \sim q$, this process
implicitly defines a set of marginal probabilities $\{p_t\}_t$,
such that $p_t$ is the marginal distribution of $x_t$.
Following the notation of the previous section,
we can write the entire process as
\begin{align}
q = p_1
\overset{v_1}{\longrightarrow}
p_{(1-\dt)} 
\overset{v_{1-\dt}}{\longrightarrow}
p_{(1-2\dt)}
\cdots
\overset{v_{\dt}}{\longrightarrow}
p_{0} 
\end{align}
which we shorten as
\[
p_1 \overset{v}{\hookrightarrow} p_0.
\]

A \emph{conditional flow} $\{\vtxo\}$ is a flow that transports $q$ to a delta distribution $\delta_{x_0}$,
for some point $x_0 \in \R^d$.
That is,
\[
q \flowto{\vxo} \delta_{x_0}.
\]
For example, in Section~\ref{sec:ddim} we 
constructed conditional flows
which transported the standard Gaussian distribution
to a single point (Equation~\ref{eqn:vtz}).
We call these \emph{conditional} flows because we will
later consider flows that are random variables,
equal to $\vtxo$ where $x_0$ is sampled from a certain distribution\footnote{
Comparing our notation to \citet{lipman2023flow}:
Our conditional vector fields $\vtxo$ 
are denoted as $u_t(\cdot \mid x_0)$ in \citet{lipman2023flow}.
Moreover, \citet{lipman2023flow} reverses time
and lets $t=0$ be the base distribution, and $t=1$
the target distribution.
We let $t=0$ be the target distribution, to be consistent
with the notation of DDPMs and DDIMs in the previous section.}.

A \emph{pointwise flow} (denoted $\Tab{a}{b}$ for points $a, b \in \R^d$)
refers to any flow between two delta distributions:
\[
\delta_{a} \flowto{\Tab{a}{b}} \delta_{b}.
\]

Finally, we often want to
compute the trajectory of just a
single point transported along a flow.
For flow $\{V_t\}$ and initial point $x_1$, we write
\begin{align}
x_t \gets \mathrm{RunFlow}(V, x_1, t)
\end{align}
to denote the result of transporting point $x_1$ along the flow $V$,
up to time $t$.
In other words\footnote{In continuous time, RunFlow is the solution
of the flow ODE (Equation~\ref{eqn:v_ode}) at time $t$, with boundary condition $x_1$.}, RunFlow is the result of
the iteration in Equation~\eqref{eqn:iterx} run from initial point $x_1$, up to time $t$.

Table~\ref{tab:notation} collects 
all of the notation in this section.

\clearpage
\newpage
\begin{fullwidth}
\begin{table*}[t]
\renewcommand{\arraystretch}{1.5} %
\centering
\classiccaptionstyle
    \begin{tabular}{rp{8cm}}
         \toprule
         $p$ & Target distribution \\
         $q$ & Base (or ``source'') distribution \\
        $\{v_t\}_t$, or $v$ & Flow: a collection of vector fields
        $v_t: \R^d \to \R^d$ indexed by time $t$. \\
        $A \flowto{v} B$ & The flow $\{v_t\}_t$ transports distribution $A$ to distribution $B$. \\
        $v(A)$ & The result of transporting distribution $A$ along flow $\{v_t\}$. So, $A \flowto{v} v(A)$. \\
        $x_t \gets \rflow(v, x_1, t)$ &
        The result of transporting point $x_1$ along the flow $v$,
        up to time $t$. In other words, the solution of
        the ODE $dx_t/dt = -v_t(x_t)$ at time $t=0$,
        with boundary condition $x_1$ at $t=1$. \\
        $\vxo$ & A conditional flow which transports $q$ to $\delta_{x_0}$. \\
        $\Tab{a}{b}$ & A pointwise flow which transports $\delta_a$ to $\delta_b$. \\
        $v^*$ & Marginal flow from $q$ to $p$. \\
        \bottomrule
    \end{tabular}
    \caption{Notation}
    \label{tab:notation}
\end{table*}
\end{fullwidth}
\nopagebreak
\begin{figure*}[b]
    \centering
    \classiccaptionstyle
    \includegraphics[width=0.95\linewidth]{figs/cfm_circle_linear.pdf}
    \caption{Example of a conditional flow which generates the point $x_0$.
    Gray arrows depict the flow vector field $\vtxo$, at different times $t$.
    The leftmost \mbox{$(t=1)$} plot shows samples from the base distribution $q$, which is
    uniform over an annulus. Subsequent plots show these samples transported by the flow,
    at intermediate times $t$. The final \mbox{$(t=0)$} plot shows
    all points collapsed to the target $x_0$.
    This particular $x_0$ happens to be one point on the spiral distribution of Figure~\ref{fig:cfm_demo}.
    }
    \label{fig:circle-cfm-old}
\end{figure*}


\clearpage
\newpage
\subsection{Method: Conditional Flow Matching}
\label{sec:cfm}

To construct a conditional flow-matching generative model
for a distribution $p(x)$, we need to specify:
\begin{enumerate}
    \item A base distribution $q(x)$, from which we can easily sample.
    This does not need to be Gaussian.
    \item 
    For every $x_0$ in the support of $p$,
    a conditional flow $\{\vtxo\}_t$ which generates point $x_0$
    from base distribution $q$:
    $$
    \forall x_0 \in \textrm{Supp}(p): ~~q \flowto{\vxo} \delta_{x_0}.
    $$
    
    We should be able to explicitly compute
    the conditional flow vector $\vtxo(z)$ at any point $z$.
\end{enumerate}

We have considerable flexibility in the second step.
It is often easy to construct a conditional flow
for a specific point $x_0$, since it
only needs to generate a single point.
We saw one example of a conditional flow in our analysis of DDIM
in Section~\ref{sec:ddim-vf}, where we constructed a flow that collapses a Gaussian distribution
to a single point at its mean.
Figure~\ref{fig:circle-cfm} illustrates another example of a conditional flow in $\R^2$,
where the base distribution $q(x)$ is not Gaussian.


Given the above,
we want to somehow construct an overall \emph{marginal flow}
$\{v_t^*\}$ which generates the entire distribution:
\begin{align}
\label{eqn:vstarflow}
q \flowto{v^*} p 
= \E_{x_0 \sim p}[\delta_{x_0}],
\end{align}
where we have slightly abused notation by writing
the distribution $p$ as a mixture of dirac deltas.
Our ``gas combination'' example from Section~\ref{sec:ddim}
tells us how to do this: following Equation~\eqref{eqn:vel_combo},
to determine $v_t^*(x_t)$, we should
take a weighted-average of all conditional velocities $\vtxo(x_t)$,
weighted by the probability that point $x_t$ was generated by 
initial point $x_0$. This is equivalent to the following conditional expectation:
\begin{align}
\label{eqn:vexp}
v_t^*(x_t) =
\E_{x_0 \sim p(x_0 \mid x_t)}[ \vtxo(x_t) ].
\end{align}
The flow $v^*$ defined above
will satisfy Equation~\eqref{eqn:vstarflow}, as desired\footnote{
The ``gas combination'' analogy used to derive Equation~\eqref{eqn:vexp}
is formalized below, as Lemma~\ref{lem:master-flow}.}.
As an example, the conditional flow in Figure~\ref{fig:circle-cfm}
generates a single point $x_0$,
but when such flows are combined for all $x_0$ in spiral distribution,
it yields a marginal flow in Figure~\ref{fig:cfm_demo},
that generates the entire spiral.


The only remaining problem is: how do we learn $v^*$ from samples?
We cannot directly compute $v^*$ from Equation~\eqref{eqn:vexp},
because it requires sampling from $p(x_0 \mid x_t)$ for a given point $x_t$.
Instead, we will take advantage of the same trick
from DDPM: it is enough for us to be able to sample from the joint distribution $(x_0, x_t)$,
and then solve a regression problem.
Similar to DDPM, the conditional expectation function in Equation~\eqref{eqn:vexp}
can be written as a regressor\footnote{The result in Line~\ref{line:cfm_argmin} corresponds to Theorem 2 in \citet{lipman2023flow}.}:

\begin{align}
v^*_t(x_t)
&:=
\E_{x_0 \sim p(x_0 \mid x_t)}[ \vtxo(x_t) ] \\
&=
\E_{x_0}[ \vtxo(x_t) \mid x_t ] \\
\implies 
v_t^* &=\argmin_{f: \R^d \to \R^d}
~~\E_{(x_0, x_t)}
||f(x_t) -  \vtxo(x_t)||_2^2.
\label{line:cfm_argmin}
\end{align}
Line~\eqref{line:cfm_argmin} follows from the previous line by the 
generic fact that for any distribution on $(x, y)$,
we have
$\argmin_{f} \E ||f(x) - y||^2 = \E[y \mid x]$.

This gives us a recipe for learning the marginal flow $v^*_t$ by optimization:
we first sample a pair $(x_0, x_t)$,
then optimize an L2 loss between our model's prediction 
$f(x_t)$ and the conditional flow vector $\vtxo(x_t)$.
Note that we can easily sample from $(x_0, x_t)$:
we first sample a train point $x_0 \sim p$,
then sample an endpoint $x_1 \sim q$, and 
then output $\mathrm{RunFlow}(v^{[x_0]}, x_1, t)$.
We will see explicit examples of training and sampling in the Pointwise Flows section below
(Section~\ref{sec:ptwise-flow}),
which generalizes conditional flows.

\subsection{The Flow Combining Lemma}
To be precise, we will state the ``gas combination'' analogy of Section~\ref{sec:ddim}
as a self-contained lemma.
Readers willing to believe the above derivation of Equation~\eqref{eqn:vexp}
may skip this subsection.

The motivation for this lemma is, we need a way of combining flows:
of taking several different flows and producing a single ``effective flow'',
such that this new flow has the same effect as running each of the individual flows ``in parallel''.
As a warm-up, suppose we have $n$ different flows, each with their own 
initial and final distributions $q_i, p_i$:
\begin{align*}
q_1 &\flowto{v^{(1)}} p_1 \\
q_2 &\flowto{v^{(2)}} p_2 \\
&\vdots \\
q_n &\flowto{v^{(n)}} p_n
\end{align*}
We can imagine these as the flow of $n$ different gases
(similar to Figure~\ref{fig:gas}),
where gas $i$ has initial density $q_i$ and final density $p_i$.
Now we want to construct an overall flow $v^*$
which takes the average initial-density to the average final-density:
\[
\E_{i \in [n]}[q_i]
\flowto{v^*}
\E_{i \in [n]}[p_i]
\]
To construct $v^*_t(x_t)$, we must take an average of the individual
vector fields $v^{(i)}$, weighted by the 
probability mass the $i$-th flow places on $x_t$, at time $t$.
(This is exactly analogous to Figure~\ref{fig:gas}).

This construction is formalized in Lemma~\ref{lem:master-flow}.
There, instead of averaging over just a finite set of flows, we are allowed
to average over any \emph{distribution} over flows.




\begin{mdframed}[nobreak]
\begin{lemma}[Flow Combining Lemma]
\label{lem:master-flow}
Let $\Gamma$ be an arbitrary distribution over flows.
Each flow vector-field $v = \{v_t\}$ comes with an associated initial
distribution $q_v$,
so $\Gamma$ is a joint distribution 
over pairs $(v, q_v)$.

For fixed $t \in [0, 1]$, consider the joint distribution over
$(x_1, x_t, w_t) \in (\R^d)^3$ generated by:
\begin{align*}
(v, q_v) &\sim \Gamma \\
x_1 &\sim q_v \\
x_t &:= \mathrm{RunFlow}(v, x_1, t) \\
w_t &:= v_t(x_t).
\end{align*}
Then, taking all expectations w.r.t. this joint distribution, the flow $v^*$ defined as
\begin{align}
v^*_t(x_t) &:= \E[w_t \mid x_t] \\
&= \E[v_t(x_t) \mid x_t] 
\end{align}
is known as the \emph{marginal flow for $\Gamma$}, and satisfies:
\begin{align}
\E[q_v]
\flowto{v^*}
\E[ v(q_v) ].
\end{align}

\end{lemma}
\end{mdframed}



\subsection{Method: Pointwise Flows}
\label{sec:ptwise-flow}

Earlier in Conditional Flow Matching (Section~\ref{sec:cfm}),
we saw how to construct a flow between two distributions ($q \flowto{} p$)
out of ``building blocks'' of simpler flows,
from $q$ to a \emph{single arbitrary point} ($q \flowto{} \delta_{x_0}$).
Here we will reduce this even further, 
so we only need to use as building-blocks flows which transport 
\emph{points to points} ($\delta_{x_1} \flowto{} \delta_{x_0}$).
\pnote{todo, more explicit about the symmetry going on}




\paragraph{Warm-up.}

Here is the idea: suppose for all pairs of points
$(x_1, x_0)$,
we have an explicit flow $\Tab{x_1}{x_0}$ which transports
source point $x_1$ to target point $x_0$.
That is, 
\[
\forall x_0 \in \mathrm{Supp}(p),~
x_1 \in \mathrm{Supp}(q):
\quad
\delta_{x_1} \flowto{\Tab{x_1}{x_0}} \delta_{x_0}.
\label{eqn:pt_flow}
\]
We call these \emph{pointwise flows}, since they transport single points.





We can use these pointwise flows to construct a conditional flow
which transports the distribution $q \flowto{} \delta_{x_0}$,
by combining\footnote{In words, if we know how to transport each source point to a target point,
then this defines how to transport the entire \emph{source distribution} to the target point.}
the flows
$\Tab{x_1}{x_0}$
for different source points $x_1 \sim q$.
The gas combination analogy (formalized as Lemma~\ref{lem:master-flow})
tell us exactly how to do this.
Specifically, the flow $\vtxo$ defined as
\begin{align}
\vtxo(x_t) 
&:= \E_{x_1 \sim p(x_1 \mid x_0, x_t)}[\Tab{x_1}{x_0}_t(x_t)]  \\
&= \E_{x_1 \mid x_t}[\Tab{x_1}{x_0}_t(x_t) \mid x_t] 
\end{align}
is a valid conditional flow which generates $x_0$, meaning
\[
q = \E_{x_1 \sim q}[\delta_{x_1}]
\flowto{\vxo}
\delta_{x_0}.
\]

For example, in Figure~\ref{fig:circle-cfm} each source point (in blue)
individually travels on a straight line from its initial position to the target point $x_0$.
These are the trajectories of the \emph{pointwise flows}.
Together these pointwise flows transport the entire
circle distribution to the point $x_0$, thus defining the \emph{conditional flow} for $x_0$.



With the conditional flows $\vxo$ in hand, we can use our previous result (Equation~\ref{eqn:vexp})
to construct a marginal flow $v^*$:
\begin{align}
\label{eqn:cfm_ptwise_to_marg}
v^*_t(x_t) &:= \E_{x_0 \mid x_t}[ \vtxo(x_t) \mid x_t ] \\
&= \E_{x_0, x_1 \mid x_t}[\Tab{x_1}{x_0}_t(x_t) \mid x_t] %
\label{line:ptwise-marg}
\end{align}
This flow $v^*$ transports the entire base distribution to the entire
target distribution ($q \flowto{v^*} p$), as desired.
This concludes our construction of an overall marginal flow
from individual pointwise flows.

Stepping back, in the preceding steps we have taken the pointwise flows
($\delta_{x_1} \flowto{} \delta_{x_0}$), and combined flows 
by averaging over both source point $x_1 \sim q$ and target point $x_0 \sim p$,
to yield an overall flow between source and target distributions $q \flowto{} p$.
In fact, we could have done this directly, instead of first constructing a conditional flow.
The resulting method is cleaner to present, and slightly more general --- we describe it below.


\paragraph{Full Construction.}
We now present the full method of pointwise flow matching.
Given a target distribution $p$, a pointwise flow is defined by the following ingredients,
which we are free to specify:

\begin{enumerate}
    \item A source distribution $q$.
    \item A \emph{coupling} $\Pi_{q, p}$ between distributions $q$ and $p$.
    This coupling specifies how to jointly sample pairs $(x_1, x_0)$ of source and target points,
    such that $x_0$ is marginally distributed as $p$, and $x_1$ as $q$.
    We must be able to sample efficiently from this coupling.
    \item For all pairs $(x_1, x_0)$, a \emph{pointwise flow} $\Tab{x_1}{x_0}$
    which transports $x_1$ to $x_0$.
\[
    \forall x_0 \in \mathrm{Supp}(p),~ x_1 \in \mathrm{Supp}(q):
\quad \delta_{x_1} \flowto{\Tab{x_1}{x_0}} \delta_{x_0}.
\]
We must be able to efficiently compute the vector field $\Tab{x_1}{x_0}_t$
at all points.\footnote{
One way to get a pointwise flow between $x_1, x_0$ is to first define
a \emph{path} $X: [0, 1] \to \R^d$ with endpoints $X(0) = x_0, X(1)=x_1$,
then let the flow vector field be the velocity 
along this path: $\Tab{x_1}{x_0}_t(x_t) := -\nicefrac{dX}{dt}\vert_t$.
}
\end{enumerate}
These ingredients determine a marginal vector field $v^*$
such that
\[
q \flowto{v^*} p.
\]
Specifically, by Lemma 2 we have
\begin{align}
v^*_t(x_t) &:= \E_{x_0, x_1 \mid x_t}[\Tab{x_1}{x_0}_t(x_t) \mid x_t] 
\end{align}
where the expectation is w.r.t. the joint distribution distribution:
\begin{align*}
(x_1, x_0) &\sim \Pi_{q,p} \\
x_t &:= \mathrm{RunFlow}(\Tab{x_1}{x_0}, x_1, t).
\end{align*}

\newthought{During training,} we want to learn the vector field $v_t^*$
given samples from $\Pi$.
Since $v_t^*$ is a conditional expectation,
it can be learnt via a regression loss just as we saw in Conditional Flow Matching.
\begin{align}
v_t^* 
&=\argmin_{f: \R^d \to \R^d} ~~\E_{(x_0, x_1, x_t)}
||f(x_t) -  \Tab{x_1}{x_0}_t(x_t)||_2^2.
\label{eqn:cfm_ptwise}
\end{align}
In words, Equation~\eqref{eqn:cfm_ptwise}
says that to compute the loss of a model $f_\theta$ for a fixed time $t$, we should:
\begin{enumerate}
    \item Sample source and target points $(x_1, x_0)$ according to our coupling $\Pi$
    \item Compute the deterministic point $x_t$, by running the pointwise flow
    $\Tab{x_1}{x_0}$ starting from point $x_1$ up to time $t$.
    \item Evaluate the model's prediction at $x_t$, as $f_\theta(x_t)$.
    Evaluate the deterministic vector $\Tab{x_1}{x_0}_t(x_t)$. 
    Then compute L2 loss between these two quantities. 
\end{enumerate}

To sample from the trained model (our estimate of $v_t^*$),
we first sample a source point $x_1 \sim q$, then transport it along the learnt flow
to a target sample $x_0$. Pseudocode listings ~\ref{alg:fm_train} and ~\ref{alg:fm_gen}
give the explicit procedures for training and sampling from flow-based models.



\SetKwComment{Comment}{// }{}
\begin{fullwidth}
\begin{minipage}[t]{0.47\linewidth}
\begin{algorithm}[H]
\DontPrintSemicolon
\caption{Flow-matching train loss, generic pointwise flow \textcolor{red}{[or linear flow]} }\label{alg:fm_train}
\KwIn{Mini-batch of samples $S$, Neural network $f_\theta$}
\KwData{Sample-access to coupling $\Pi_{q, p}$;
Pointwise flows $\{\Tab{x_1}{x_0}_t\}$ for all $x_1, x_0$.}
\KwOut{Stochastic loss $L$}
$(x_1, x_0) \gets \mathrm{Sample}( \Pi_{q,p} )$ \;
$t \gets \textrm{Unif}[0, 1]$ \;
$x_t \gets \mathcolor{red}{\underbrace{\mathcolor{black}{\mathrm{RunFlow}(\Tab{x_1}{x_0}, x_1, t)}}_{tx_1 + (1-t)x_{0}}}$  \;
$L \gets \Big\Vert f_\theta(x_t, t) -  \mathcolor{red}{\underbrace{\mathcolor{black}{\Tab{x_1}{x_0}_t(x_t)}}_{(x_0 - x_1)}} \Big\Vert_2^2$ \;
\Return $L$
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.47\linewidth}
\begin{algorithm}[H]
\DontPrintSemicolon
\caption{Flow-matching sampling}\label{alg:fm_gen}
\KwIn{Trained model $f_\theta$}
\KwData{Sample-access to base distribution $q$; step-size $\dt$.}
\KwOut{Sample from target distribution $p$.}
$x_1 \gets \mathrm{Sample}(q)$ \;
\For{$t=1,~(1-\dt),(1-2\dt), \dots, \dt$}{
$x_{t-\dt} \gets x_t + f_\theta(x_t, t)\dt$ \;
}
\Return $x_0$
\end{algorithm}
\end{minipage}

\end{fullwidth}

\subsection{Example: Rectified Flows}
\pnote{TODO}

\subsection{Example: DDIM as a Flow}
\pnote{TODO; don't read.}

The flow matching framework above can formally capture DDIM trajectories (of Section~\ref{sec:ddim}) as a special case.
This should not be surprising, since our analysis of DDIM was already inspired by flows, but we 
describe the exact correspondence here for completeness.
The only notable difference from Section~\ref{sec:ddim} is:
we will adopt the continuous-time discretization from Section~\ref{sec:flow-notation},
where $t \in [0, 1]$, rather than the discrete time indices $t \in \N$ used in Section~\ref{sec:ddim}.

Given a target distribution $p_0$, we think of DDIM as a flow from
initial distribution $p_1 := p_0 \star \cN(0, \sigma^2_q)$
to 
final distribution $p_0$.
The marginal distributions at intermediate times are $p_t = p_0 \star \cN(0, t\sigma_q^2)$.

The DDIM update implements the following marginal flow (when $\dt \to 0$):
\begin{align}
\label{eqn:v_ddim}
    v^{\textrm{ddim}}_t(x_t) 
    &= \frac{1}{2t} \E[x_0 - x_t \mid x_t] 
\end{align}
\pnote{todo: footnote, it is possible to show this is the continuous-time limit of...} \anote{The result is also given in eq \ref{eq:simple_pf_ode} as the continuous-time limit of our simple discrete DDIM (though we have to go through SDEs to get there...)  }

This marginal flow can be equivalently constructed 
in several ways: from conditional flows, or from pointwise flows.

We took the conditional flow approach in Section~\ref{sec:ddim},
where we designed flows that transport a Gaussian to a single point at its mean.
Specifically, each conditional flow $\vtxo$ transports:
\[
\delta_{x_0} \star \cN(0, \sigma_q^2) \flowto{\vxo} \delta_{x_0}
\]
where the LHS is equal to $\cN(x_0, \sigma_q^2)$.
One flow that implements this is:
\begin{align}
    \vtxo(x_t) &:=
    \frac{1}{2t} \E[x_0 - x_t \mid x_t, x_0] \\
    &= \frac{1}{2t} (x_0 - x_t)
\end{align}
\pnote{then, applying the gas lemma,...}

\pnote{todo: will add more details below:}

The DDIM flow can also be constructed from pointwise flows, along with a special coupling.
Specifically, consider:
\begin{itemize}
    \item Pointwise flows:
    \[
    \label{eqn:ptwise_ddim}
    \Tab{x_1}{x_0}(x_t)
    := \frac{1}{2t}(x_0 - x_t).
    \]
    This pointwise flow generates the trajectory\footnote{
    By Separable Equations method:
    \begin{align*}
        \frac{dx_t}{dt} &= -\frac{1}{2t} (x_0 - x_t) \\
        \implies \frac{\frac{dx_t}{dt}}{x_t - x_0} &= \frac{1}{2t} \\
        \implies \int \frac{1}{x_t - x_0} dx &= \int \frac{1}{2t} dt, 
        \text{ since } \frac{dx_t}{dt} dt = dx \\
        \implies \log(x_t - x_0) &= \log \sqrt{t} + c \\
        c &= \log(x_1 - x_0) \text{ (boundary cond.)}\\
        \implies \log(x_t - x_0) &= \log \sqrt{t} (x_1 - x_0)  \\
        \implies x_t - x_0 &= \sqrt{t} (x_1 - x_0)\\
    \end{align*}
    }:
    \[
    \label{eqn:ptwise_traj}
    x_t = x_0 + (x_1 - x_0)\sqrt{t}
    \]
    which is like a ``linear flow with time scaling as $\sqrt{t}$.''
    
    Furthermore, by taking time-derivatives of Equation~\eqref{eqn:ptwise_traj},
    we see the flow in Line~\eqref{eqn:ptwise_ddim}
    generates the same trajectory as the flow:
    \[
    \label{eqn:ptwise_ddim2}
    \Tab{x_1}{x_0}_{(\textrm{lin})}(x_t)
    = \frac{1}{2\sqrt{t}}(x_0 - x_1).
    \]
    \item Coupling: Joint distribution $(x_0, x_1)$ generated by:
    $$x_0 \sim p_0; \quad x_1 \gets x_0 + \cN(0, \sigma_q^2).$$
    Note, this is the ``DDPM coupling.''
\end{itemize}

\pnote{todo: write out that linear flows and DDIM are basically the same; the only difference is the initial distribution / coupling, and the time-rescaling.}

\begin{tcolorbox}[colback=gray!10,colframe=black!80,halign=left,title=DDIM vs Linear Flows]

The following lemma states that the trajectories defined by variance-exploding DDIM
and linear flows are equivalent, provided the linear flow uses the same coupling between
initial and terminal distributions as variance-exploding DDPM.


\begin{lemma}[DDIM vs Linear Flows]
\newcommand{\pddim}{p^{\textrm{ddim}}}

Let $p$ be an arbitrary target distribution.
Let $\{x_t\}_t$ be the joint distribution defined by the
DDPM forward process applied to $p$, so the marginal distribution of $x_t$
is $p_t = p \star \cN(0, t\sigma_q^2)$.

Let $x^* \in \R^d$ be an arbitrary initial point.
Consider the following two deterministic trajectories:
\begin{enumerate}
    \item The trajectory $\{y_t\}_t$ of the continuous-time DDIM flow,
    with respect to target distribution $p_0$ and base distribution $p_1$,
    when started at initial point $y_1 = x^*$.
    
    That is, $y_t$ is the solution to the following ODE
    \begin{align}
    \frac{dy_t}{dt} &= -v^{\mathrm{ddim}}(y_t) \\
    &= -\frac{1}{2t} \E_{x_0 \mid x_t}[x_0 - x_t \mid x_t=y_t] 
    \end{align}
    with boundary condition $y_1$ at $t=1$.

    \item The trajectory $\{z_t\}_t$ of linear flow
    between distribution $p_0$ and base distribution $p_1$,
    using the DDPM-coupling $p(x_0, x_1)$, and initial point $z_1 = x^*$.

\end{enumerate}
These two trajectories are identical up to time-rescaling:
\begin{align}
\forall t: \quad
y_t = z_{\sqrt{t}}
\end{align}
\end{lemma}

This setup differs from standard linear flows
in two ways:
\begin{enumerate}
    \item The base distribution here is $p_1 = p \star \cN(0, \sigma_q^2)$,
    as opposed to pure noise $\cN(0, \sigma_q^2)$.
    \item The coupling used is the DDPM coupling,
    as opposed to the standard independent coupling.
\end{enumerate}
However, notice that for large terminal noise $\sigma_q$,
both of these differences decay to $0$.

\end{tcolorbox}


\newcommand{\ssig}{{\sigma^2}}

\pnote{this section is WIP}

\pnote{nb: linear flows are NOT equivalent to ddim (even for same terminal distribution),
and also not the same as Lipman.}

\pnote{DDIM is equivalent to linear flows with a certain coupling.
In particular, with the diffusion joint distribution on $(x_0, x_t, x_1)$.
In other words, linear flows with a aprtiuar coupling, and with a non-constant speed.}


\subsubsection*{One-point Example}
Let's first work out the details when $p_0 = \delta_{0}$.

For linear flows, we have a joint distribution over $(x_0, x_t, x_1)$ where
$x_0 = 0$, $x_1 \sim \cN(0, \sigma_q^2)$, and 
\begin{align}
x_t &= t x_1 + (1-t)x_0 \\
&= t x_1
\end{align}
Since we have $x_1 \sim \cN(0, \sigma_q^2)$,
the marginal distribution of $x_t$ for linear flows is:
\[
p^{\textrm{lin}}_t = \cN(0, t^2\sigma_q^2).
\]
Compare this to the marginal distribution of DDIM:
\[
p^{\textrm{ddim}}_t = \cN(0, t \sigma_q^2).
\]

So, linear flows and DDIMs have the same marginal
distributions (up to time-rescaling),
but linear flows are ``slower'' than DDIM when $t$ is small.



\pnote{nb:
- only needs to define the reverse process, and only for one point.
- computational: why the expectations make training easy.
}



\begin{fullwidth}
\begin{table}
    \begin{tabular}{lllll}
    \toprule
    Method & Coupling & Pointwise Flow & Pointwise Trajectory & Conditional Flow  \\
    \midrule
    DDIM & - & - & - & - \\
    Rectified Flow & - & - & - & - \\
    \bottomrule
    \end{tabular}
    \label{tab:flows}
\end{table}
\end{fullwidth}

\subsection{Other Resources}

\pnote{todo: flow matching is natural, but not much research yet. }

\begin{itemize}
    \item \citet{albergo2023stochastic} define the framework of \emph{stochastic interpolants}, which is a generalization of CFMs.
    See their work for more rigorous mathematical formalism.
    \item See \citet{stark2024dirichlet} 
    for an interesting example of non-standard flows.
    They derive a generative model for discrete spaces by embedding
    into a continuous space (the probability simplex), then 
    constructing a special flow on these simplices.
    \item \pnote{manifold diffusions}
    \item \pnote{text diffusion}
\end{itemize}



\subsection*{FIXME stuff we might or might not need}
\anote{Just stashing this stuff here in case we need it}
As a final connection, recall the PF-ODE (\ref{eqn:pf_ode}) corresponding to the general SDE (\ref{eq:general_sde}): 
$$\frac{dx}{dt} = \tilde f(x, t).$$ 
This means that $\tilde f$ is a vector field that generates the diffusion path. We can use this to derive the conditional vector field corresponding to our simple diffusion, (similar to \citet{lipman2023flow} equation 17):
\begin{align*}
    v_t(x) &= \tilde f(x) \equiv \frac{1}{2} \sigma_q^2 \nabla_x \log p_t(x) \mathnote{\ref{eq:simple_pf_ode}}\\
    p_t(x|x_0) &= \cN(x| x_0, \sigma_t) 
    \implies \nabla_x \log p_t(x) = \frac{1}{\sigma_t^2} (x - x_0) \\
    \implies \vtxo(x) \dt &= \frac{1}{2t} (x - x_0)
\end{align*}

==> sec_practical_old.tex <==
\clearpage
\newpage
\section{Elucidating Design Choices (old)}
\label{sec:practical}

\hnote{wip here}

In the previous sections, we discussed the basic formulation and intuition of diffusion models. In this section, we will present more general formulations of Gaussian diffusion and highlight the various design choices available. We can define the discrete forward Gaussian diffusion process more generally as:
\begin{align}
p(x_t \mid x_{t-1}) &= \cN(x_t; s_t x_{t-1}, \sigma_t^2 I)  \\
x_t &= s_t x_{t-1} + \sigma_t \epsilon \text{, where } \epsilon \sim \cN(0, I)
\end{align}

Here, $s_t$ represents a time-dependent scaling factor and $\sigma^2_t$ represents a time-dependent noise level. In the previous examples we have assumed $s_t = 1$ and $\sigma^2_t$ is monotonically increasing with $t$. This is often referred to as the \emph{variance-exploding} formulation. However, we can make different choices for the scaling the variance schedules, which we will show correspond to different SDEs. The only constraint is that the signal-to-noise ratio\footnote{We can define the signal-to-noise ratio as $\text{SNR}(t) = s_t^2 / \sigma_t^2$. We want to use a sequence of $s_t$ and $\sigma_t$ such that $\text{SNR}(t) < \text{SNR}(t+1)$ for all $t$.} needs to be monotonically increasing with $t$, which would define increasingly noisier versions of $x_0$.


Due to the linearity of the Gaussian diffusion model, we can sample $x_t$ directly from $x_0$. We can represent the cumulative scaling coefficient as a function depending on the time step $t$ as $s(t)$, and similarly represent the cumulative noise coefficient as $\sigma(t)$. We can now represent $p(x_t \mid x_0)$ as:
\begin{align}
p(x_t \mid x_0) &= \cN(x_{t}; s(t) x_0, s(t)^2 \sigma(t)^2 I)
\end{align}





As we saw in Section xxx, a more general way to define diffusion models is as a continuous time process. 
We can write this as a stochastic differential equation (SDE):
\begin{align}
dx &= f(t) x dt + g(t) dw
\end{align}

Song et al defines the probability flow ODE as:
\begin{align}
dx &= [f(t) x - 0.5 g(t)^2 \nabla_{x} \log p_t({x})]\,dt
\end{align}





How do we connect the SDE formulation with the scaling ($s(t)$) and noise ($\sigma(t)$) functions we've just defined? Intuitively, notice that the SDE represents an instaneous change, while the $p(x_t \mid x_0)$ formulation represents a cumulative move from $x_0$. Thus, we can connect $s(t)$ to $f(t)$ and $\sigma(t)$ to $g(t)$ as follows:
\begin{align}
s(t) = \exp\left(\int_0^t f(\xi) d\xi\right), \quad \text{and} \quad \sigma(t) = \sqrt{\int_0^t \frac{g(\xi)^2}{s(\xi)^2} d\xi}.
\end{align}

Conversely, we can rearrange the equations to show that:
\begin{align}
f(t) = \dot{s}(t)/s(t), \quad \text{and} \quad g(t) = s(t) \sqrt{2 \dot{\sigma}(t) \sigma(t)},
\end{align}
where $\dot{s}(t) = ds(t)/dt$ represents the time derivative of $s(t)$ and similarly for $\dot{\sigma}(t) = d\sigma(t)/dt$.

With these definitions, we can rewrite $p_t$ as:


\begin{align}
p_t(x) &= \int_{\R^d} p_{data}(x_0)  p(x_t \mid x_0) \,dx_0\\
&= \int_{\R^d} p_{data}(x_0) [\cN(x_{t}; s(t) x_0, s(t)^2 \sigma(t)^2 I)]\,dx_0\\
&= s(t)^{-d}  \int_{\R^d} p_{data}(x_0) [\cN(x_{t} / s(t); x_0, \sigma(t)^2 I)]\,dx_0\\
&= s(t)^{-d} \int_{\R^d} p_{data}(x_0)  [\cN(x_{t} / s(t) - x_0; 0, \sigma(t)^2 I)]\,dx_0
\end{align}

We can represent equation 31 as the convolution of $p_{data}(x)$ and $\cN(0, \sigma(t)^2I)$ evaluated at $x_t / s(t)$.\footnote{The convolution of two independent PDFs $f$ and $g$ is defined as $f*g(z) = \int_{\R^d}f(x) g(z-x)\,dx$. The convolution represents the distribution of $f+g$. In diffusion terms, this represents the distribution we get through adding Gaussian noise to the data distribution. We can see that $p_t$ is thus a distribution arising from $p_{data}$ + $\cN(0, \sigma_t^2)$.} We can define $p(x; \sigma)$ as $p(x; \sigma) = p_{data} * \cN(0, \sigma^2I)$. Thus, we can write:
\begin{align}
p_t(x) &= s(t)^{-d} p(x_t / s(t); \sigma(t))
\end{align}


Pulling everything together, we can insert these terms into the probability flow ODE formulation\footnote{The $s(t)^{-d}$ term can be omitted because it is not a function of $x$ and has no effect in the log derivative term.}:
\begin{align}
dx &= \left[ f(t) x - \frac{1}{2} g(t)^2 \nabla_x \log p(x / s(t); \sigma(t)) \right] dt \\
&= \left[ \frac{\dot{s}(t)}{s(t)} x - \frac{1}{2} \left[ s(t) \sqrt{2 \dot{\sigma}(t) \sigma(t)}\right] ^2 \nabla_x \log p(x / s(t); \sigma(t)) \right] dt \\
&= \left[ \frac{\dot{s}(t)}{s(t)} x - \frac{1}{2} 2 s(t)^2 \dot{\sigma}(t) \sigma(t) \nabla_x \log p(x / s(t); \sigma(t)) \right] dt \\
&= \left[ \frac{\dot{s}(t)}{s(t)} x - s(t)^2 \dot{\sigma} (t) \sigma(t) \nabla_x \log p(x / s(t); \sigma(t)) \right] dt
\end{align}


So what have we learned? Every specification of a probability flow ODE can be represented by equation 39. This means that every probability flow ODE is fully determined by the functions $s(t)$ and $\sigma(t)$. Moreover, in practice we discretize the ODE, and the schedule we use is another design choice.
\hnote{add properties of s and sigma}

Let's now see some examples of different diffusion specifications. One way is to add noise to unscaled $x$ at each step. This equates to setting $s(t) = 1$. In this case, we have:
\begin{align}
dx = - \dot{\sigma}(t) \sigma(t) \nabla_x \log p(x; \sigma(t)) dt
\end{align}

If we define $\sigma(t) = \sqrt{t}$, then we have
\begin{align}
dx &= - 0.5 \nabla_x \log p(x; \sigma(t)) dt
\end{align}
\hnote{where did the $\sigma^2$ go}
\anote{I think this is correct as the ODE for the VE case; if you rewrite the score in terms of $E[x_0 - x_t|x_t]$ you will get a factor of $\frac{1}{\sigma^2} = \frac{1}{t}$, see eq \ref{eq:score_vs_expt_contin}.}

This equates to the setting where 
\[p(x_t \mid x_{t-1}) = \cN(x_{t-1}, tI)\]

Setting $s(t) = 1$ gives a \textit{variance-exploding} process, where the variance of $x_t$ explodes as $t \rightarrow \infty$. \hnote{practically we can normalize? where?}

Another commonly used model is the \textit{variance-preserving} formulation introduced in DDPM. We define an arithmetic sequence schedule 
\[\beta(t) = (\beta_{max} - \beta_{min}) t + \beta_{min}\]

\hnote{why do we need $\beta_{max}$ and $\beta_{min}$?}
\anote{I believe $\beta_{max}$ and $\beta_{min}$ are chosen in conjunction with the number of steps $T$ to ensure that the schedule has endpoints close to (but not exactly) zero and 1.}

and define $f(t) = -\frac{1}{2}\beta(t)$ and $g(t) = \sqrt{\beta(t)}$. Moreover, let us define the integral of $\beta(t)$ as 
\begin{align}
    \alpha(t) &= \int_0^t \beta(\xi) d\xi\\
    &= \frac{1}{2}(\beta_{max} - \beta_{min}) t^2 + \beta_{min}t
\end{align}
Then, we have $s(t) = e^{-\frac{1}{2} \alpha(t)}$ and $\sigma(t) = \sqrt{e^{\alpha(t)} - e^{\alpha(0)}}$. We can further simplify these equations as $s(t) = 1/\sqrt{\sigma(t)^2 + 1}$.
Pulling everything together, the variance-preserving formulation implies the following diffusion process\footnote{For small $x$, $\sqrt{1-x} \approx 1 - \frac{1}{2}x$. Thus, we can show that for small $\Delta t$:
\begin{align*}
x(t + \Delta t) &= \sqrt{1 - \beta(t + \Delta t)\Delta t} \, x(t) + \sqrt{\beta(t + \Delta t)\Delta t} \, z(t)\\
&\approx x(t) - \frac{1}{2} \beta(t + \Delta t)\Delta t \, x(t) + \sqrt{\beta(t + \Delta t)\Delta t} \, z(t)\\
&\approx x(t) - \frac{1}{2} \beta(t)\Delta t \, x(t) + \sqrt{\beta(t)\Delta t} \, z(t)
\end{align*}
}:
\begin{align}
x_t &= \sqrt{1-\beta(t)} x_{t-1} + \sqrt{\beta(t)} \epsilon
\end{align}
\begin{align}
p(x_t \mid x_0) &= \cN(x_t; \frac{x_0}{\sqrt{\sigma(t)^2 + 1}}, \frac{\sigma(t)^2}{\sigma(t)^2+1}I)
\end{align}

The corresponding SDE is:
\begin{align}
dx &= - \frac{1}{2} \beta(t)x dt + \sqrt{\beta(t)} dw
\end{align}

The corresponding probability flow ODE is:
\begin{align}
dx &= [- \frac{1}{2} \beta(t) x - \frac{1}{2} \beta(t) \log p(x / s(t); \sigma(t))]\,dt
\end{align}

\hnote{add stuff on what we know about how to choose the various schedules}





\subsection{Scaling and noise schedule}

The noise schedule typically refers to $\sigma(t)$, which defines the amount of noise added at time $t$. This is often coupled with the \emph{sampling} schedule, which defines the distribution we use to sample $t$. In practice, we typically sample $t \sim U(0,1)$ from a uniform distribution, and focus the design choices on $\sigma(t)$. 

Kingma et al introduced a general formulation of the diffusion loss objective, and showed that many popular diffusion objectives are special cases of the following with a particular choice of weighting function $w(\lambda_t)$:
\begin{align}
\mathcal{L}_w (\mathbf{x}) = \frac{1}{2} \mathbb{E}_{t\sim U(0,1),\epsilon\sim \mathcal{N}(0,I)} \left[ w(\lambda_t) \cdot \left( - \frac{d\lambda}{dt} \cdot \| \hat{\epsilon}_\theta(\mathbf{z}_t; \lambda_t) - \epsilon \|_2^2 \right) \right]
\end{align}

Here, $\lambda$ is the log-SNR, which can be written as $\lambda = \log \frac{s_t^2}{\sigma_t^2}$ for $p(x_t \mid x_{t-1}) = \cN(s_t x_{t-1}, \sigma_t^2 I)$. \anote{my reading of Kingma is that the SNR is actually in terms of the mean/variance of $x_t$, not the conditional? also I think this gets confusing when combined with Karras because in Karras the SNR would just be $\sigma(t)$} With a monotonic choice of the weighting function, this objective corresponds to the ELBO under data augmentation with additive Gaussian noise\footnote{This is essentially a lower bound on the log-likelihood of noise-perturbed data.}. This means that optimizing this objective will also optimize our model for $p_{data}(x)$. \hnote{check} Interestingly, some of the best performing methods do not use monotonic weighting functions\footnote{They showed that this loss can be equivalently written as:
\begin{align}
\mathcal{L}_w (\mathbf{x}) = \frac{1}{2} \int_{\lambda_{min}}^{\lambda_{max}} w(\lambda_t) \cdot \mathbb{E}_{\epsilon\sim \mathcal{N}(0,I)} [ \| \hat{\epsilon}_\theta(\mathbf{z}_t; \lambda_t) - \epsilon \|_2^2 ] d\lambda
\end{align}

This means that for the loss objective, only $\lambda_{min}$ and $\lambda_{max}$ matter and the loss is invariant to the choice of the noise schedule. However, since we train the models with Monte Carlo sampling in practice, the noise schedule affects the variance of this estimator.}.

\hnote{insert figure for different weighting functions}

Since we start from no noise and end with random noise, we can intuitively see that the noise schedule determines how much the model focuses on different noise levels. Indeed, Kingma showed that the noise distribution acts as an importance sampling distribution for estimating the loss. 

During training, we sample $t$ uniformly then compute $\lambda = f_t(\lambda)$. This gives us a cumulative density function $F(\lambda) = 1-f_t^{-1}(\lambda)$ and a corresponding PDF $p(\lambda) = -1/(d\lambda / dt)$. Thus we can formalize the importance sampling as follows:

\begin{align}
\mathcal{L}_w (\mathbf{x}) = \frac{1}{2} \mathbb{E}_{\lambda \sim p(\lambda),\epsilon\sim \mathcal{N}(0,I)} \left[ \frac{w(\lambda_t)}{p(\lambda_t)} \cdot \| \hat{\epsilon}_\theta(\mathbf{z}_t; \lambda_t) - \epsilon \|_2^2 \right]
\end{align}

For models that are defined as continuous-time models (e.g. with a SDE), any sampling method is approximate. The noise schedule can influence the amount of discretization error. The magnitude of the discretization error scales proportionately to the curvature of $dx(t)/dt$. \citet{karras2022elucidating} argues that the best choice for these functions is $s(t) = 1$ and $\sigma(t) = t$. With these choices, equation 45 becomes 
\[dx =( x - D(x;t))/t\]
\hnote{how?}
\anote{Like this, I think \footnote{
\begin{align*}
    \sigma(t) &= t \implies \dot{\sigma}(t) \sigma(t) = t \\
    dx & %
    = -t \nabla \log p(x_t) dt \\
    x_t &= \cN(x_0, t^2) \overset{Tweedie}{\implies} \E[x_0 | x_t] = x_t + t^2 \log p(x_t) \\
    \implies dx &= (x_t - \E[x_0 | x_t]) / t
\end{align*}
}
Note also that the choices $s=1$, $\sigma(t) = t$ correspond to $f=0$,  $g(t)=\sqrt{2t}$
}

This means that the trajectory always points to the optimal denoiser output.


Compared to monotonic schedules that puts the highest weight on the highest noise levels, non-monotonic weighting functions tend to put the highest weight at medium noise levels. Intuitively, at low noise levels the denoising objective becomes relatively easy, and at high noise levels there is very little information and the optimal denoiser should just predict the mean of the dataset. Thus, reducing the weighting at those noise levels can help the model focus on the bulk of the problem. Other intuitions in the image space suggest that it may be better to focus on the low frequency features in an image and less on the high frequency features. \citet{choi2022perception} suggests that medium noise levels require the model to reconstruct the features most sensitive to visual perception. \hnote{todo: elaborate}




The optimal noise level also depends on the amount of signal and redundancy in the data. For example, high resolution images will be easier to denoise at the same noise level than low resolution images, since correlation between nearby pixels tend to increase with image size. \citet{chen2023importance} showed that different image resolution has different optimal noise schedules, and it is difficult to predict the optimal one due to the number of hyperparameters involved.

\hnote{mention learned noise schedules?}








\subsection{Sources of Error}
\pnote{todo}





==> tufte-handout-local.tex <==


\RequirePackage{etoolbox}
\makeatletter
\newif\if@tufte@margtab\@tufte@margtabfalse
\AtBeginEnvironment{margintable}{\@tufte@margtabtrue}
\AtEndEnvironment{margintable}{\@tufte@margtabfalse}
\newcommand{\classiccaptionstyle}{%
    \long\def\@caption##1[##2]##3{%
        \par
        \addcontentsline{\csname ext@##1\endcsname}{##1}%
        {\protect\numberline{\csname the##1\endcsname}{\ignorespaces ##2}}%
        \begingroup
        \@parboxrestore
        \if@minipage
        \@setminipage
        \fi
        \normalsize
        \@makecaption{\csname fnum@##1\endcsname}{\ignorespaces ##3}\par
        \endgroup}
    \long\def\@makecaption##1##2{%
        \vskip\abovecaptionskip
        \sbox\@tempboxa{\@tufte@caption@font##1: ##2}%
        \ifdim \wd\@tempboxa >\hsize
        \@tufte@caption@font\if@tufte@margtab\@tufte@caption@justification\fi##1: ##2\par
        \else
        \global \@minipagefalse
        \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
        \fi
        \vskip\belowcaptionskip}
      \setcaptionfont{\normalfont}
    \let\caption\@tufte@orig@caption%
    \let\label\@tufte@orig@label}
\makeatother

\newenvironment{pagefigure}{%
    \begin{figure*}[p]
    \classiccaptionstyle
  }{\end{figure*}}



\titleformat{\section}[hang]
{\normalfont\huge\bfseries}{\thesection}{1em}{}[]





\makeatletter
\renewcommand{\maketitle}{%
  \newpage
  \global\@topnum\z@%
  \begin{fullwidth} %
  \begingroup
    \setlength{\parindent}{0pt}%
    \setlength{\parskip}{4pt}%
    \let\@@title\@empty
    \let\@@author\@empty
    \let\@@date\@empty
    \gdef\@@title{\LARGE\textsc{\@title}\par}%
    \gdef\@@author{\large\itshape\@author\par}%
    \gdef\@@date{\large\itshape\@date\par}%
    \@@title
    \@@author
    \@@date
  \endgroup
  \end{fullwidth}
  \thispagestyle{plain}%
  \tuftebreak%
  \@afterindentfalse\@afterheading%
}
\makeatother


